Concept-Monitor: Understanding DNN training through individual neurons

In this work, we propose a general framework called Concept-Monitor to help demystify the black-box DNN training processes automatically using a novel unified embedding space and concept diversity metric. Concept-Monitor enables human-interpretable visualization and indicators of the DNN training processes and facilitates transparency as well as deeper understanding on how DNNs develop along the during training. Inspired by these findings, we also propose a new training regularizer that incentivizes hidden neurons to learn diverse concepts, which we show to improve training performance. Finally, we apply Concept-Monitor to conduct several case studies on different training paradigms including adversarial training, fine-tuning and network pruning via the Lottery Ticket Hypothesis

==> table/concept-evo-comparison.tex <==
\begin{table*}[h]
\centering
\scalebox{0.49}{
\begin{tabular}{c|ccccc}
\toprule
\textbf{Method} & \thead{Training\\Free}  & \thead{Automatic \\ Concepts} & \thead {Embedding space \\ Tracking} & \thead {Embedding space \\ anchors} & \thead {Flexible probing \\ dataset} \\ \midrule 
\makecell{ConceptEvo} & No & No & \bf{Yes} & No & No \\
\makecell{\algoname{}} & \bf{Yes} & \bf{Yes} & \bf{Yes} & \bf{Yes} & \bf{Yes} \\
\bottomrule
\end{tabular}}
\caption{Comparison between our method and a recent work Concept-Evo \citep{park2022conceptevo}. \tuomas{Do we need this table? Maybe appendix}}
\label{tab:comparison}
\end{table*}

==> table/method_strength_example.tex <==
\begin{table}[b]
\centering
\scalebox{0.88}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Property / \\ Method \end{tabular} & \begin{tabular}[c]{@{}l@{}}Training\\ free \end{tabular} & \begin{tabular}[c]{@{}l@{}}Provides \\ concepts \end{tabular} & \begin{tabular}[c]{@{}l@{}} \\ Embedding  \\ space tracking\end{tabular} & \begin{tabular}[c]{@{}l@{}}Embedding  \\ space anchors \end{tabular} & \begin{tabular}[c]{@{}l@{}} \\ information \\ of neuron \\ activations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Generative \\ natural \\ language \\ descriptions\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Concept \\ Evolution \\ (\cite{park2022conceptevo})\end{tabular} & Yes & No & No & \textbf{Yes} & \textbf{Yes} & No  \\ \midrule
\begin{tabular}[c]{@{}l@{}}\algoname \\ \textbf{(Ours)} \end{tabular}  & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} & No & No \\ 
\bottomrule
\end{tabular}}
\caption{Comparison of existing automated neuron labeling methods and whether they have certain desirable properties. \lily{need to update this table, and what's the column: describe more than top few images?}}
\label{tab:method_strengths}
\end{table}
